SemanticLock: An authentication method for mobile devices using semantically-linked images

We introduce SemanticLock, a single factor graphical authentication solution for mobile devices. SemanticLock uses a set of graphical images as password tokens that construct a semantically memorable story representing the user`s password. A familiar and quick action of dragging or dropping the images into their respective positions either in a \textit{continous flow} or in \textit{discrete} movements on the the touchscreen is what is required to use our solution. The authentication strength of the SemanticLock is based on the large number of possible semantic constructs derived from the positioning of the image tokens and the type of images selected. Semantic Lock has a high resistance to smudge attacks and it equally exhibits a higher level of memorability due to its graphical paradigm. In a three weeks user study with 21 participants comparing SemanticLock against other authentication systems, we discovered that SemanticLock outperformed the PIN and matched the PATTERN both on speed, memorability, user acceptance and usability. Furthermore, qualitative test also show that SemanticLock was rated more superior in like-ability. SemanticLock was also evaluated while participants walked unencumbered and walked encumbered carrying "everyday" items to analyze the effects of such activities on its usage.

==> semantic_lock_pwdIcon_eval.tex <==
\section{Semantic-Lock password icon selection and practical space evaluation}

In the design of our Semantic-lock system, our initial intention is to avoid any implicitly induced biases in the researchers selection of the password icons. In general, security experts have observed that an authentication systems \textit{theoretical password space} is never optimally achieved during practical usage and there is a need to determine the actual \textit{practical password space} that suggests the ecological validity of such authentication system. Experiments by Deluca et al \cite{DeLuca:2010:CSP:1753326.1753490} and Chiasson et al \cite{Cha:2017:BGA:3052973.3052989} observed this outcome within their results. A preliminary user study of associating icons indicated  a need to define a process for the selection of a set of unbiased password icons for our Semantic-lock system. We define two stages of experiment to achieve the above stated objectives, and implemented these stages with two different groups of participants. The output of the analysis of the dataset collected in the first stage was utilized during the second stage. No demographic data was collect from the participant during these stages.
\subsection{STAGE 1 : Acquisition of Independent password Icons}
%\subsubsection{Initial Icon base set selections}
Our initial process was to provide a set of 40 icons that were drawn from various categories and genres. We pointedly avoided icons that had major gender significant colors, cultural, national and religious relevance. On the other hand, we also inserted icons that were abstract in context to ensure a balance of our base set of icons.\\
\par 
Our participants were then presented with a web-based interface that displayed these icons on a 10 by 4 grid; with each icon randomly positioned in different grid-cells during every selection session to prevent locational bias. Participants were required to create 10 sets of two \textit{"icons-pairs"} that they believed were related by dragging these icons into the provide \textit{`pairboxes`} (see figure XXX). Each participation was allowed multiple iterations.\\
\par
Although our experimental methodology was designed for our participants to select icons that they deemed related, we analyzed the 1039 collected \textit{pair-datasets} to extract 6 icons that were the least intrinsically related. These \textit{"non-intrinsically"} related icons were used in our next stage of the experiment. 



\subsection{STAGE 2: Evaluation of practical password space}
Every authentication scheme has an entropy and the strength of such entropy is determined by the size of the theoretical password space. However, researchers perform  experiments and also use large-scale actual user-data to evaluate the true value of the \textit{practical password space} of their authentication systems. In this stage of our experiment we presented a web-based interface displaying the six derived \textit{non-intrinsically related}  password icons on a 9 by 6 celled grid to our participants. Our participants were required to create several semantic passwords with the password icons by dragging a choosen icon to the left, top, right or bottom position of an associated stationary icon. (see fig XXXX) . Using the resulting data we were able to make some determinations about the data as discussed below.
\subsubsection{Password Icon distribution}
\subsubsection{Password Icon pair distribution}
\subsubsection{Password Icon-pair position distribution}
